PANOC-lite: A simpler and more efficient algorithm for composite minimization

This work introduces a simple and efficient linesearch method for composite minimization that accelerates proximal-gradient iterations with fast Newton-type directions. Our algorithm is based on simple operations and only requires the standard proximal-gradient oracle, similar to PANOC and ZeroFPR, provided that the nonsmooth term is convex. Noteworthy improvements include a cheaper backtracking procedure, in the sense that no additional gradients need to be evaluated, and an enlarged range of permitted stepsizes. Global subsequential convergence and local superlinear convergence are established under conventional assumptions by considering a novel merit function which is less expensive to evaluate than alternatives like the forward-backward envelope. Finally, the proposed approach is validated on model predictive control problems with collision avoidance constraints, as well as on the LIBSVM and CUTEst benchmarks.

==> tikz/bicycle/mpc_metrics_hermans_bicycle_ss2p_32_N30_mem50_warmfalse_f_plus_grad_evals.tex <==
% Recommended preamble:
% \usetikzlibrary{arrows.meta}
% \usetikzlibrary{backgrounds}
% \usepgfplotslibrary{patchplots}
% \usepgfplotslibrary{fillbetween}
% \pgfplotsset{%
%     layers/standard/.define layer set={%
%         background,axis background,axis grid,axis ticks,axis lines,axis tick labels,pre main,main,axis descriptions,axis foreground%
%     }{
%         grid style={/pgfplots/on layer=axis grid},%
%         tick style={/pgfplots/on layer=axis ticks},%
%         axis line style={/pgfplots/on layer=axis lines},%
%         label style={/pgfplots/on layer=axis descriptions},%
%         legend style={/pgfplots/on layer=axis descriptions},%
%         title style={/pgfplots/on layer=axis descriptions},%
%         colorbar style={/pgfplots/on layer=axis descriptions},%
%         ticklabel style={/pgfplots/on layer=axis tick labels},%
%         axis background@ style={/pgfplots/on layer=axis background},%
%         3d box foreground style={/pgfplots/on layer=axis foreground},%
%     },
% }

\begin{tikzpicture}[/tikz/background rectangle/.style={fill={rgb,1:red,1.0;green,1.0;blue,1.0}, fill opacity={1.0}, draw opacity={1.0}}, show background rectangle]
\begin{axis}[point meta max={nan}, point meta min={nan}, legend cell align={left}, legend columns={1}, title={}, title style={at={{(0.5,1)}}, anchor={south}, font={{\fontsize{14 pt}{18.2 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}, align={center}}, legend style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, line width={1}, solid, fill={rgb,1:red,1.0;green,1.0;blue,1.0}, fill opacity={1.0}, text opacity={1.0}, font={{\fontsize{8 pt}{10.4 pt}\selectfont}}, text={rgb,1:red,0.0;green,0.0;blue,0.0}, cells={anchor={center}}, at={(0.98, 0.98)}, anchor={north east}}, axis background/.style={fill={rgb,1:red,1.0;green,1.0;blue,1.0}, opacity={1.0}}, anchor={north west}, xshift={1.0mm}, yshift={-1.0mm}, width={150.4mm}, height={99.6mm}, scaled x ticks={false}, xlabel={MPC time step}, x tick style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, opacity={1.0}}, x tick label style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, opacity={1.0}, rotate={0}}, xlabel style={at={(ticklabel cs:0.5)}, anchor=near ticklabel, at={{(ticklabel cs:0.5)}}, anchor={near ticklabel}, font={{\fontsize{11 pt}{14.3 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}}, xmajorgrids={true}, xmin={0.129999999999999}, xmax={30.87}, xticklabels={{$5$,$10$,$15$,$20$,$25$,$30$}}, xtick={{5.0,10.0,15.0,20.0,25.0,30.0}}, xtick align={inside}, xticklabel style={font={{\fontsize{8 pt}{10.4 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}}, x grid style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={0.1}, line width={0.5}, solid}, axis x line*={left}, x axis line style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, line width={1}, solid}, scaled y ticks={false}, ylabel={Function + gradient evaluations}, y tick style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, opacity={1.0}}, y tick label style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, opacity={1.0}, rotate={0}}, ylabel style={at={(ticklabel cs:0.5)}, anchor=near ticklabel, at={{(ticklabel cs:0.5)}}, anchor={near ticklabel}, font={{\fontsize{11 pt}{14.3 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}}, ymode={log}, log basis y={10}, ymajorgrids={true}, ymin={225.63046277892175}, ymax={12890.49343860012}, yticklabels={{$10^{3}$,$10^{4}$}}, ytick={{1000.0,10000.0}}, ytick align={inside}, yticklabel style={font={{\fontsize{8 pt}{10.4 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}}, y grid style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={0.1}, line width={0.5}, solid}, axis y line*={left}, y axis line style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, line width={1}, solid}, colorbar={false}]
    \addplot[color={rgb,1:red,0.0;green,0.6056;blue,0.9787}, name path={25}, draw opacity={1.0}, line width={1}, solid]
        table[row sep={\\}]
        {
            \\
            1.0  11496.0  \\
            2.0  9661.0  \\
            3.0  5604.0  \\
            4.0  5974.0  \\
            5.0  5120.0  \\
            6.0  5626.0  \\
            7.0  4791.0  \\
            8.0  5726.0  \\
            9.0  4885.0  \\
            10.0  4224.0  \\
            11.0  4813.0  \\
            12.0  3472.0  \\
            13.0  3379.0  \\
            14.0  2976.0  \\
            15.0  2771.0  \\
            16.0  2027.0  \\
            17.0  1619.0  \\
            18.0  2216.0  \\
            19.0  2897.0  \\
            20.0  1977.0  \\
            21.0  1722.0  \\
            22.0  1236.0  \\
            23.0  1284.0  \\
            24.0  1220.0  \\
            25.0  1123.0  \\
            26.0  721.0  \\
            27.0  670.0  \\
            28.0  976.0  \\
            29.0  643.0  \\
            30.0  616.0  \\
        }
        ;
    \addlegendentry {panoc}
    \addplot[color={rgb,1:red,0.8889;green,0.4356;blue,0.2781}, name path={26}, draw opacity={1.0}, line width={1}, solid]
        table[row sep={\\}]
        {
            \\
            1.0  8380.0  \\
            2.0  8040.0  \\
            3.0  4663.0  \\
            4.0  4599.0  \\
            5.0  7309.0  \\
            6.0  3601.0  \\
            7.0  3143.0  \\
            8.0  4373.0  \\
            9.0  2899.0  \\
            10.0  2961.0  \\
            11.0  2883.0  \\
            12.0  2255.0  \\
            13.0  2269.0  \\
            14.0  1935.0  \\
            15.0  1193.0  \\
            16.0  953.0  \\
            17.0  1033.0  \\
            18.0  1859.0  \\
            19.0  1805.0  \\
            20.0  1253.0  \\
            21.0  2921.0  \\
            22.0  1085.0  \\
            23.0  875.0  \\
            24.0  3032.0  \\
            25.0  1419.0  \\
            26.0  1389.0  \\
            27.0  667.0  \\
            28.0  681.0  \\
            29.0  403.0  \\
            30.0  429.0  \\
        }
        ;
    \addlegendentry {zfpr}
    \addplot[color={rgb,1:red,0.2422;green,0.6433;blue,0.3044}, name path={27}, draw opacity={1.0}, line width={1}, solid]
        table[row sep={\\}]
        {
            \\
            1.0  4015.0  \\
            2.0  3581.0  \\
            3.0  2865.0  \\
            4.0  2860.0  \\
            5.0  2636.0  \\
            6.0  2304.0  \\
            7.0  2238.0  \\
            8.0  2209.0  \\
            9.0  2040.0  \\
            10.0  1931.0  \\
            11.0  2389.0  \\
            12.0  1640.0  \\
            13.0  1612.0  \\
            14.0  1408.0  \\
            15.0  1044.0  \\
            16.0  864.0  \\
            17.0  753.0  \\
            18.0  928.0  \\
            19.0  1038.0  \\
            20.0  860.0  \\
            21.0  858.0  \\
            22.0  748.0  \\
            23.0  651.0  \\
            24.0  561.0  \\
            25.0  430.0  \\
            26.0  320.0  \\
            27.0  299.0  \\
            28.0  253.0  \\
            29.0  316.0  \\
            30.0  257.0  \\
        }
        ;
    \addlegendentry {zfpr\_pp}
\end{axis}
\end{tikzpicture}


==> tikz/bicycle/mpc_metrics_hermans_bicycle_ss2p_32_N30_mem50_warmtrue_f_plus_grad_evals.tex <==
% Recommended preamble:
% \usetikzlibrary{arrows.meta}
% \usetikzlibrary{backgrounds}
% \usepgfplotslibrary{patchplots}
% \usepgfplotslibrary{fillbetween}
% \pgfplotsset{%
%     layers/standard/.define layer set={%
%         background,axis background,axis grid,axis ticks,axis lines,axis tick labels,pre main,main,axis descriptions,axis foreground%
%     }{
%         grid style={/pgfplots/on layer=axis grid},%
%         tick style={/pgfplots/on layer=axis ticks},%
%         axis line style={/pgfplots/on layer=axis lines},%
%         label style={/pgfplots/on layer=axis descriptions},%
%         legend style={/pgfplots/on layer=axis descriptions},%
%         title style={/pgfplots/on layer=axis descriptions},%
%         colorbar style={/pgfplots/on layer=axis descriptions},%
%         ticklabel style={/pgfplots/on layer=axis tick labels},%
%         axis background@ style={/pgfplots/on layer=axis background},%
%         3d box foreground style={/pgfplots/on layer=axis foreground},%
%     },
% }

\begin{tikzpicture}[/tikz/background rectangle/.style={fill={rgb,1:red,1.0;green,1.0;blue,1.0}, fill opacity={1.0}, draw opacity={1.0}}, show background rectangle]
\begin{axis}[point meta max={nan}, point meta min={nan}, legend cell align={left}, legend columns={1}, title={}, title style={at={{(0.5,1)}}, anchor={south}, font={{\fontsize{14 pt}{18.2 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}, align={center}}, legend style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, line width={1}, solid, fill={rgb,1:red,1.0;green,1.0;blue,1.0}, fill opacity={1.0}, text opacity={1.0}, font={{\fontsize{8 pt}{10.4 pt}\selectfont}}, text={rgb,1:red,0.0;green,0.0;blue,0.0}, cells={anchor={center}}, at={(0.98, 0.98)}, anchor={north east}}, axis background/.style={fill={rgb,1:red,1.0;green,1.0;blue,1.0}, opacity={1.0}}, anchor={north west}, xshift={1.0mm}, yshift={-1.0mm}, width={150.4mm}, height={99.6mm}, scaled x ticks={false}, xlabel={MPC time step}, x tick style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, opacity={1.0}}, x tick label style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, opacity={1.0}, rotate={0}}, xlabel style={at={(ticklabel cs:0.5)}, anchor=near ticklabel, at={{(ticklabel cs:0.5)}}, anchor={near ticklabel}, font={{\fontsize{11 pt}{14.3 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}}, xmajorgrids={true}, xmin={0.129999999999999}, xmax={30.87}, xticklabels={{$5$,$10$,$15$,$20$,$25$,$30$}}, xtick={{5.0,10.0,15.0,20.0,25.0,30.0}}, xtick align={inside}, xticklabel style={font={{\fontsize{8 pt}{10.4 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}}, x grid style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={0.1}, line width={0.5}, solid}, axis x line*={left}, x axis line style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, line width={1}, solid}, scaled y ticks={false}, ylabel={Function + gradient evaluations}, y tick style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, opacity={1.0}}, y tick label style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, opacity={1.0}, rotate={0}}, ylabel style={at={(ticklabel cs:0.5)}, anchor=near ticklabel, at={{(ticklabel cs:0.5)}}, anchor={near ticklabel}, font={{\fontsize{11 pt}{14.3 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}}, ymode={log}, log basis y={10}, ymajorgrids={true}, ymin={43.34917920355674}, ymax={13524.961966336256}, yticklabels={{$10^{2}$,$10^{3}$,$10^{4}$}}, ytick={{100.0,1000.0,10000.0}}, ytick align={inside}, yticklabel style={font={{\fontsize{8 pt}{10.4 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}}, y grid style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={0.1}, line width={0.5}, solid}, axis y line*={left}, y axis line style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, line width={1}, solid}, colorbar={false}]
    \addplot[color={rgb,1:red,0.0;green,0.6056;blue,0.9787}, name path={25}, draw opacity={1.0}, line width={1}, solid]
        table[row sep={\\}]
        {
            \\
            1.0  11496.0  \\
            2.0  9529.0  \\
            3.0  4871.0  \\
            4.0  4911.0  \\
            5.0  4706.0  \\
            6.0  4023.0  \\
            7.0  3819.0  \\
            8.0  4751.0  \\
            9.0  3814.0  \\
            10.0  3681.0  \\
            11.0  4530.0  \\
            12.0  2775.0  \\
            13.0  2693.0  \\
            14.0  2547.0  \\
            15.0  2651.0  \\
            16.0  1667.0  \\
            17.0  1625.0  \\
            18.0  2021.0  \\
            19.0  1808.0  \\
            20.0  1617.0  \\
            21.0  1155.0  \\
            22.0  725.0  \\
            23.0  782.0  \\
            24.0  553.0  \\
            25.0  81.0  \\
            26.0  93.0  \\
            27.0  84.0  \\
            28.0  84.0  \\
            29.0  84.0  \\
            30.0  60.0  \\
        }
        ;
    \addlegendentry {panoc}
    \addplot[color={rgb,1:red,0.8889;green,0.4356;blue,0.2781}, name path={26}, draw opacity={1.0}, line width={1}, solid]
        table[row sep={\\}]
        {
            \\
            1.0  8380.0  \\
            2.0  5996.0  \\
            3.0  3231.0  \\
            4.0  4155.0  \\
            5.0  4649.0  \\
            6.0  2751.0  \\
            7.0  2279.0  \\
            8.0  2615.0  \\
            9.0  2317.0  \\
            10.0  2303.0  \\
            11.0  2711.0  \\
            12.0  1939.0  \\
            13.0  1695.0  \\
            14.0  1599.0  \\
            15.0  1003.0  \\
            16.0  1071.0  \\
            17.0  833.0  \\
            18.0  859.0  \\
            19.0  785.0  \\
            20.0  815.0  \\
            21.0  751.0  \\
            22.0  447.0  \\
            23.0  447.0  \\
            24.0  398.0  \\
            25.0  55.0  \\
            26.0  51.0  \\
            27.0  59.0  \\
            28.0  57.0  \\
            29.0  53.0  \\
            30.0  57.0  \\
        }
        ;
    \addlegendentry {zfpr}
    \addplot[color={rgb,1:red,0.2422;green,0.6433;blue,0.3044}, name path={27}, draw opacity={1.0}, line width={1}, solid]
        table[row sep={\\}]
        {
            \\
            1.0  4015.0  \\
            2.0  3462.0  \\
            3.0  2410.0  \\
            4.0  2504.0  \\
            5.0  2351.0  \\
            6.0  1902.0  \\
            7.0  1914.0  \\
            8.0  1985.0  \\
            9.0  1964.0  \\
            10.0  1723.0  \\
            11.0  2016.0  \\
            12.0  1487.0  \\
            13.0  1382.0  \\
            14.0  1298.0  \\
            15.0  893.0  \\
            16.0  836.0  \\
            17.0  764.0  \\
            18.0  785.0  \\
            19.0  819.0  \\
            20.0  777.0  \\
            21.0  573.0  \\
            22.0  379.0  \\
            23.0  455.0  \\
            24.0  345.0  \\
            25.0  60.0  \\
            26.0  56.0  \\
            27.0  60.0  \\
            28.0  58.0  \\
            29.0  57.0  \\
            30.0  61.0  \\
        }
        ;
    \addlegendentry {zfpr\_pp}
\end{axis}
\end{tikzpicture}


==> tikz/quadcopter/mpc_metrics_quadcopter_ss2p_32_N30_mem50_warmfalse_f_plus_grad_evals.tex <==
% Recommended preamble:
% \usetikzlibrary{arrows.meta}
% \usetikzlibrary{backgrounds}
% \usepgfplotslibrary{patchplots}
% \usepgfplotslibrary{fillbetween}
% \pgfplotsset{%
%     layers/standard/.define layer set={%
%         background,axis background,axis grid,axis ticks,axis lines,axis tick labels,pre main,main,axis descriptions,axis foreground%
%     }{
%         grid style={/pgfplots/on layer=axis grid},%
%         tick style={/pgfplots/on layer=axis ticks},%
%         axis line style={/pgfplots/on layer=axis lines},%
%         label style={/pgfplots/on layer=axis descriptions},%
%         legend style={/pgfplots/on layer=axis descriptions},%
%         title style={/pgfplots/on layer=axis descriptions},%
%         colorbar style={/pgfplots/on layer=axis descriptions},%
%         ticklabel style={/pgfplots/on layer=axis tick labels},%
%         axis background@ style={/pgfplots/on layer=axis background},%
%         3d box foreground style={/pgfplots/on layer=axis foreground},%
%     },
% }

\begin{tikzpicture}[/tikz/background rectangle/.style={fill={rgb,1:red,1.0;green,1.0;blue,1.0}, fill opacity={1.0}, draw opacity={1.0}}, show background rectangle]
\begin{axis}[point meta max={nan}, point meta min={nan}, legend cell align={left}, legend columns={1}, title={}, title style={at={{(0.5,1)}}, anchor={south}, font={{\fontsize{14 pt}{18.2 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}, align={center}}, legend style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, line width={1}, solid, fill={rgb,1:red,1.0;green,1.0;blue,1.0}, fill opacity={1.0}, text opacity={1.0}, font={{\fontsize{8 pt}{10.4 pt}\selectfont}}, text={rgb,1:red,0.0;green,0.0;blue,0.0}, cells={anchor={center}}, at={(0.98, 0.98)}, anchor={north east}}, axis background/.style={fill={rgb,1:red,1.0;green,1.0;blue,1.0}, opacity={1.0}}, anchor={north west}, xshift={1.0mm}, yshift={-1.0mm}, width={150.4mm}, height={99.6mm}, scaled x ticks={false}, xlabel={MPC time step}, x tick style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, opacity={1.0}}, x tick label style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, opacity={1.0}, rotate={0}}, xlabel style={at={(ticklabel cs:0.5)}, anchor=near ticklabel, at={{(ticklabel cs:0.5)}}, anchor={near ticklabel}, font={{\fontsize{11 pt}{14.3 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}}, xmajorgrids={true}, xmin={0.129999999999999}, xmax={30.87}, xticklabels={{$5$,$10$,$15$,$20$,$25$,$30$}}, xtick={{5.0,10.0,15.0,20.0,25.0,30.0}}, xtick align={inside}, xticklabel style={font={{\fontsize{8 pt}{10.4 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}}, x grid style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={0.1}, line width={0.5}, solid}, axis x line*={left}, x axis line style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, line width={1}, solid}, scaled y ticks={false}, ylabel={Function + gradient evaluations}, y tick style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, opacity={1.0}}, y tick label style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, opacity={1.0}, rotate={0}}, ylabel style={at={(ticklabel cs:0.5)}, anchor=near ticklabel, at={{(ticklabel cs:0.5)}}, anchor={near ticklabel}, font={{\fontsize{11 pt}{14.3 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}}, ymode={log}, log basis y={10}, ymajorgrids={true}, ymin={2090.3021862332907}, ymax={36765.64111454405}, yticklabels={{$10^{3.6}$,$10^{3.9}$,$10^{4.2}$,$10^{4.5}$}}, ytick={{3981.0717055349774,7943.282347242822,15848.931924611174,31622.776601683858}}, ytick align={inside}, yticklabel style={font={{\fontsize{8 pt}{10.4 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}}, y grid style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={0.1}, line width={0.5}, solid}, axis y line*={left}, y axis line style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, line width={1}, solid}, colorbar={false}]
    \addplot[color={rgb,1:red,0.0;green,0.6056;blue,0.9787}, name path={25}, draw opacity={1.0}, line width={1}, solid]
        table[row sep={\\}]
        {
            \\
            1.0  33900.0  \\
            2.0  32314.0  \\
            3.0  32398.0  \\
            4.0  30068.0  \\
            5.0  27137.0  \\
            6.0  26664.0  \\
            7.0  24684.0  \\
            8.0  24123.0  \\
            9.0  23945.0  \\
            10.0  17717.0  \\
            11.0  14923.0  \\
            12.0  9332.0  \\
            13.0  5286.0  \\
            14.0  5120.0  \\
            15.0  4841.0  \\
            16.0  4679.0  \\
            17.0  4327.0  \\
            18.0  3475.0  \\
            19.0  3814.0  \\
            20.0  3688.0  \\
            21.0  4183.0  \\
            22.0  4021.0  \\
            23.0  3847.0  \\
            24.0  3910.0  \\
            25.0  4043.0  \\
            26.0  3637.0  \\
            27.0  3877.0  \\
            28.0  3745.0  \\
            29.0  3850.0  \\
            30.0  3550.0  \\
        }
        ;
    \addlegendentry {panoc}
    \addplot[color={rgb,1:red,0.8889;green,0.4356;blue,0.2781}, name path={26}, draw opacity={1.0}, line width={1}, solid]
        table[row sep={\\}]
        {
            \\
            1.0  20073.0  \\
            2.0  17821.0  \\
            3.0  17759.0  \\
            4.0  17037.0  \\
            5.0  16954.0  \\
            6.0  18662.0  \\
            7.0  15502.0  \\
            8.0  16391.0  \\
            9.0  13457.0  \\
            10.0  11084.0  \\
            11.0  10283.0  \\
            12.0  8885.0  \\
            13.0  7985.0  \\
            14.0  4893.0  \\
            15.0  4117.0  \\
            16.0  3797.0  \\
            17.0  4083.0  \\
            18.0  3907.0  \\
            19.0  3371.0  \\
            20.0  3781.0  \\
            21.0  3213.0  \\
            22.0  4109.0  \\
            23.0  3527.0  \\
            24.0  3453.0  \\
            25.0  4079.0  \\
            26.0  3277.0  \\
            27.0  3315.0  \\
            28.0  2907.0  \\
            29.0  3447.0  \\
            30.0  3609.0  \\
        }
        ;
    \addlegendentry {zfpr}
    \addplot[color={rgb,1:red,0.2422;green,0.6433;blue,0.3044}, name path={27}, draw opacity={1.0}, line width={1}, solid]
        table[row sep={\\}]
        {
            \\
            1.0  14175.0  \\
            2.0  13158.0  \\
            3.0  13288.0  \\
            4.0  14184.0  \\
            5.0  13069.0  \\
            6.0  13364.0  \\
            7.0  13186.0  \\
            8.0  12254.0  \\
            9.0  13192.0  \\
            10.0  10657.0  \\
            11.0  9318.0  \\
            12.0  9711.0  \\
            13.0  6839.0  \\
            14.0  2691.0  \\
            15.0  2405.0  \\
            16.0  2598.0  \\
            17.0  2339.0  \\
            18.0  2284.0  \\
            19.0  2761.0  \\
            20.0  2425.0  \\
            21.0  2574.0  \\
            22.0  2445.0  \\
            23.0  2335.0  \\
            24.0  2523.0  \\
            25.0  2267.0  \\
            26.0  2335.0  \\
            27.0  2355.0  \\
            28.0  2546.0  \\
            29.0  2504.0  \\
            30.0  2596.0  \\
        }
        ;
    \addlegendentry {zfpr\_pp}
\end{axis}
\end{tikzpicture}


==> tikz/quadcopter/mpc_metrics_quadcopter_ss2p_32_N30_mem50_warmtrue_f_plus_grad_evals.tex <==
% Recommended preamble:
% \usetikzlibrary{arrows.meta}
% \usetikzlibrary{backgrounds}
% \usepgfplotslibrary{patchplots}
% \usepgfplotslibrary{fillbetween}
% \pgfplotsset{%
%     layers/standard/.define layer set={%
%         background,axis background,axis grid,axis ticks,axis lines,axis tick labels,pre main,main,axis descriptions,axis foreground%
%     }{
%         grid style={/pgfplots/on layer=axis grid},%
%         tick style={/pgfplots/on layer=axis ticks},%
%         axis line style={/pgfplots/on layer=axis lines},%
%         label style={/pgfplots/on layer=axis descriptions},%
%         legend style={/pgfplots/on layer=axis descriptions},%
%         title style={/pgfplots/on layer=axis descriptions},%
%         colorbar style={/pgfplots/on layer=axis descriptions},%
%         ticklabel style={/pgfplots/on layer=axis tick labels},%
%         axis background@ style={/pgfplots/on layer=axis background},%
%         3d box foreground style={/pgfplots/on layer=axis foreground},%
%     },
% }

\begin{tikzpicture}[/tikz/background rectangle/.style={fill={rgb,1:red,1.0;green,1.0;blue,1.0}, fill opacity={1.0}, draw opacity={1.0}}, show background rectangle]
\begin{axis}[point meta max={nan}, point meta min={nan}, legend cell align={left}, legend columns={1}, title={}, title style={at={{(0.5,1)}}, anchor={south}, font={{\fontsize{14 pt}{18.2 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}, align={center}}, legend style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, line width={1}, solid, fill={rgb,1:red,1.0;green,1.0;blue,1.0}, fill opacity={1.0}, text opacity={1.0}, font={{\fontsize{8 pt}{10.4 pt}\selectfont}}, text={rgb,1:red,0.0;green,0.0;blue,0.0}, cells={anchor={center}}, at={(0.98, 0.98)}, anchor={north east}}, axis background/.style={fill={rgb,1:red,1.0;green,1.0;blue,1.0}, opacity={1.0}}, anchor={north west}, xshift={1.0mm}, yshift={-1.0mm}, width={150.4mm}, height={99.6mm}, scaled x ticks={false}, xlabel={MPC time step}, x tick style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, opacity={1.0}}, x tick label style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, opacity={1.0}, rotate={0}}, xlabel style={at={(ticklabel cs:0.5)}, anchor=near ticklabel, at={{(ticklabel cs:0.5)}}, anchor={near ticklabel}, font={{\fontsize{11 pt}{14.3 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}}, xmajorgrids={true}, xmin={0.129999999999999}, xmax={30.87}, xticklabels={{$5$,$10$,$15$,$20$,$25$,$30$}}, xtick={{5.0,10.0,15.0,20.0,25.0,30.0}}, xtick align={inside}, xticklabel style={font={{\fontsize{8 pt}{10.4 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}}, x grid style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={0.1}, line width={0.5}, solid}, axis x line*={left}, x axis line style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, line width={1}, solid}, scaled y ticks={false}, ylabel={Function + gradient evaluations}, y tick style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, opacity={1.0}}, y tick label style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, opacity={1.0}, rotate={0}}, ylabel style={at={(ticklabel cs:0.5)}, anchor=near ticklabel, at={{(ticklabel cs:0.5)}}, anchor={near ticklabel}, font={{\fontsize{11 pt}{14.3 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}}, ymode={log}, log basis y={10}, ymajorgrids={true}, ymin={120.27521157499356}, ymax={54428.48043479205}, yticklabels={{$10^{3}$,$10^{4}$}}, ytick={{1000.0,10000.0}}, ytick align={inside}, yticklabel style={font={{\fontsize{8 pt}{10.4 pt}\selectfont}}, color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, rotate={0.0}}, y grid style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={0.1}, line width={0.5}, solid}, axis y line*={left}, y axis line style={color={rgb,1:red,0.0;green,0.0;blue,0.0}, draw opacity={1.0}, line width={1}, solid}, colorbar={false}]
    \addplot[color={rgb,1:red,0.0;green,0.6056;blue,0.9787}, name path={25}, draw opacity={1.0}, line width={1}, solid]
        table[row sep={\\}]
        {
            \\
            1.0  33900.0  \\
            2.0  45779.0  \\
            3.0  45074.0  \\
            4.0  34767.0  \\
            5.0  24624.0  \\
            6.0  1752.0  \\
            7.0  987.0  \\
            8.0  624.0  \\
            9.0  402.0  \\
            10.0  598.0  \\
            11.0  367.0  \\
            12.0  418.0  \\
            13.0  280.0  \\
            14.0  508.0  \\
            15.0  277.0  \\
            16.0  429.0  \\
            17.0  222.0  \\
            18.0  258.0  \\
            19.0  468.0  \\
            20.0  237.0  \\
            21.0  300.0  \\
            22.0  279.0  \\
            23.0  348.0  \\
            24.0  168.0  \\
            25.0  363.0  \\
            26.0  273.0  \\
            27.0  201.0  \\
            28.0  342.0  \\
            29.0  207.0  \\
            30.0  447.0  \\
        }
        ;
    \addlegendentry {panoc}
    \addplot[color={rgb,1:red,0.8889;green,0.4356;blue,0.2781}, name path={26}, draw opacity={1.0}, line width={1}, solid]
        table[row sep={\\}]
        {
            \\
            1.0  20073.0  \\
            2.0  36651.0  \\
            3.0  41111.0  \\
            4.0  18311.0  \\
            5.0  14112.0  \\
            6.0  363.0  \\
            7.0  891.0  \\
            8.0  237.0  \\
            9.0  363.0  \\
            10.0  247.0  \\
            11.0  231.0  \\
            12.0  247.0  \\
            13.0  287.0  \\
            14.0  209.0  \\
            15.0  293.0  \\
            16.0  191.0  \\
            17.0  247.0  \\
            18.0  299.0  \\
            19.0  203.0  \\
            20.0  327.0  \\
            21.0  175.0  \\
            22.0  333.0  \\
            23.0  207.0  \\
            24.0  331.0  \\
            25.0  253.0  \\
            26.0  147.0  \\
            27.0  143.0  \\
            28.0  367.0  \\
            29.0  203.0  \\
            30.0  327.0  \\
        }
        ;
    \addlegendentry {zfpr}
    \addplot[color={rgb,1:red,0.2422;green,0.6433;blue,0.3044}, name path={27}, draw opacity={1.0}, line width={1}, solid]
        table[row sep={\\}]
        {
            \\
            1.0  14175.0  \\
            2.0  24672.0  \\
            3.0  23647.0  \\
            4.0  13725.0  \\
            5.0  10575.0  \\
            6.0  469.0  \\
            7.0  1750.0  \\
            8.0  237.0  \\
            9.0  288.0  \\
            10.0  218.0  \\
            11.0  381.0  \\
            12.0  299.0  \\
            13.0  209.0  \\
            14.0  317.0  \\
            15.0  268.0  \\
            16.0  377.0  \\
            17.0  318.0  \\
            18.0  202.0  \\
            19.0  256.0  \\
            20.0  226.0  \\
            21.0  286.0  \\
            22.0  295.0  \\
            23.0  179.0  \\
            24.0  179.0  \\
            25.0  374.0  \\
            26.0  198.0  \\
            27.0  283.0  \\
            28.0  200.0  \\
            29.0  311.0  \\
            30.0  202.0  \\
        }
        ;
    \addlegendentry {zfpr\_pp}
\end{axis}
\end{tikzpicture}

